Optimizing over Serial Dictatorships

Motivated by the success of the serial dictatorship mechanism in social choice settings, we explore its usefulness in tackling various combinatorial optimization problems. We do so by considering an abstract model, in which a set of agents are asked to act in a particular ordering, called the action sequence. Each agent acts in a way that gives her the maximum possible value, given the actions of the agents who preceded her in the action sequence. Our goal is to compute action sequences that yield approximately optimal total value to the agents (a.k.a., social welfare). We assume query access to the value $v_i(S)$ that the agent i gets when she acts after the agents in the ordered set $S$. We establish tight bounds on the social welfare that can be achieved using polynomially many queries. Even though these bounds show a marginally sublinear approximation of optimal social welfare in general, excellent approximations can be obtained when the valuations stem from an underlying combinatorial domain. Indicatively, when the valuations are defined using bipartite matchings, arborescences in directed graphs, and satisfiability of Boolean expressions, simple query-efficient algorithms yield $2$-approximations. We discuss issues related to truthfulness and show how some of our algorithms can be implemented truthfully using VCG-like payments. Finally, we introduce and study the price of serial dictatorship, a notion that provides an optimistic measure of the quality of combinatorial optimization solutions generated by action sequences.

==> additional-results.tex <==



\subsection{Longest paths}

In this section, we explore the instances of 
$\pro$ when valuations are derived from a 
complete directed graph $G$ with vertex set $[n]$, and weights $w(i \rightarrow j)$ for directed edges $i \rightarrow j$ with $i,j \in [n]$. \emph{Longest paths} in $G$ are defined as a union of (directed) disjoint paths where each node has at most one out-degree and at most one in-degree.
Given a weighted directed graph $G$, the problem is to find longest paths with maximum possible weight in $G$. We will refer the above optimization problem as $\paths$. 

Note that, in the query model of $\pro$, an algorithm can access the weights in the underlying graph $G$ via action sequences, i.e., it does not have direct access to the weights in $G$. For a node $i \in [n]$ and an ordered sequence $S$ of a subset of the remaining $n-1$ agents, we define the valuation query $v_i(S)$ as the maximum weight of a directed edge $(i \rightarrow j)$ such that its addition to the set of edges chosen by agents in $S$ is a union of paths in $G$. In particular, we have $v_i(\phi) = \max_{j \neq i} w(i \rightarrow j)$, and we call the corresponding edge as \emph{top-choice} edge of node $i$ in $G$. It is trivial to observe that for any ordered subset $S'$ of $S$, we have $v_i(S') \geq v_i(S)$, i.e., $v_i$s are monotone.

For a given instance of $\paths$ in the above query model, the goal is to find an action sequence $\pi  \in S_n$ that maximizes the sum of valuations of all agents, $\sum_{i \in [n]} v_i(\pi^i)$.
We prove that the price of serial dictatorship (PoSD) for $\paths$ is strictly greater than one (Theorem~\ref{theorem: paths SD}).

\begin{theorem} \label{theorem: paths SD}
	An optimal solution for instances of $\textsc{Longest-Paths}$ may not be produced by any action sequence of nodes. Moreover, the price of serial dictatorship for $\paths$ is at least $3/2$.
\end{theorem} 


\begin{proof}
	We construct an instance of $\textsc{Longest-Paths}$ consisting of four nodes $x_1, x_2, x_3$ and $x_4$ with following weights: $w(x_1 \rightarrow x_2) = w(x_2 \rightarrow x_3) =  w(x_3 \rightarrow x_4) = 1$; and $w(x_1 \rightarrow x_4) = w(x_2 \rightarrow x_4) = w(x_3 \rightarrow x_2) = 1+\varepsilon$. All the remaining edges have zero weight. Here, the unique optimal solution is the path $x_1 \rightarrow x_2 \rightarrow x_3 \rightarrow x_4$ having a weight of $3$, whereas any action sequence of these four nodes can achieve a value of at most $2+\varepsilon$. The price of serial dictatorship for $\textsc{Longest-Paths}$ is therefore at most $2/3$.
\end{proof}


The above lemma holds true for the problem of finding a Hamiltonian path of maximum weight.


%\section{Fairness with respect to Serial Dictatorship}


%\subsection{Maximum Cuts}

%\begin{lemma}
%There exists an algorithm that produces a $2$-approximation for a given instance of MAX-CUT using polynomially-many queries.
%\end{lemma}










